Anytime Approximate Formal Feature Attribution

Widespread use of artificial intelligence (AI) algorithms and machine learning (ML) models on the one hand and a number of crucial issues pertaining to them warrant the need for explainable artificial intelligence (XAI). A key explainability question is: given this decision was made, what are the input features which contributed to the decision? Although a range of XAI approaches exist to tackle this problem, most of them have significant limitations. Heuristic XAI approaches suffer from the lack of quality guarantees, and often try to approximate Shapley values, which is not the same as explaining which features contribute to a decision. A recent alternative is so-called formal feature attribution (FFA), which defines feature importance as the fraction of formal abductive explanations (AXp's) containing the given feature. This measures feature importance from the view of formally reasoning about the model's behavior. It is challenging to compute FFA using its definition because that involves counting AXp's, although one can approximate it. Based on these results, this paper makes several contributions. First, it gives compelling evidence that computing FFA is intractable, even if the set of contrastive formal explanations (CXp's) is provided, by proving that the problem is #P-hard. Second, by using the duality between AXp's and CXp's, it proposes an efficient heuristic to switch from CXp enumeration to AXp enumeration on-the-fly resulting in an adaptive explanation enumeration algorithm effectively approximating FFA in an anytime fashion. Finally, experimental results obtained on a range of widely used datasets demonstrate the effectiveness of the proposed FFA approximation approach in terms of the error of FFA approximation as well as the number of explanations computed and their diversity given a fixed time limit.

==> relw.tex <==
\section{Related Work} \label{sec:relw}
%%
%Interpretable decision sets are logic-based ML models that can be
%traced back to 70s and
%80s~\cite{michalski-isip69,rivest-ipl76,breiman-bk84,rivest-ml87}.
%%
%To the best of our knowledge, \cite{clark-ewsl91} proposed the first
%approach to decision sets, which were introduced as the variant of
%decision lists~\cite{rivest-ml87,clark-ml89}.
%%
%The first method making use of logic and optimization to synthesize a
%disjunction of rules that match a given dataset was proposed
%in~\cite{resende-mp92}.
%%
%Recent work~\cite{leskovec-kdd16} argued that decision sets are more
%interpretable than the other logic-based models, i.e. decision lists
%and decision trees.
%%
%This work uses smooth local search to generate a set of rules first and heuristically minimizes a
%linear combination of criteria afterwards, e.g. the size of a rule,
%the maximum number of rules, the overlap or error of the rules.
%
%Since then a number of works proposed the use of logic reasoning and
%optimization procedures to train DS
%models~\cite{ipnms-ijcar18,meel-cp18,gm19,yisb-cp20,ilsms-aaai21}
%claiming to significantly outperform the approach
%of~\cite{leskovec-kdd16} in terms of accuracy and performance.
%%
%Among those, the works closest to ours
%are~\cite{ipnms-ijcar18,yisb-cp20,ilsms-aaai21}.
%%
%They proposed SAT-based approaches to computing smallest-size decision
%sets that \emph{perfectly} agree with the training data by minimizing
%either the number of rules~\cite{ipnms-ijcar18,ilsms-aaai21} or the
%number of literals~\cite{yisb-cp20,ilsms-aaai21} used in the model.
%%
%Additionally, \cite{yisb-cp20} is capable of computing \emph{sparse}
%decisions sets that trade off training accuracy for model size.
%%
%Despite the dramatic performance increase achieved
%in~\cite{ilsms-aaai21}, all the approaches above suffer from
%scalability issues.
%
%%
%%However, this approach is not as scalable as the SAT-based
%%approach~\cite{ipnms-ijcar18} to minimizing the number of rules,
%%which is shown to be more coarse-grained.
%%%
%%Moreover, \cite{yisb-cp20} proposed the sparse alternative trading
%%off its accuracy for smaller number of literals used to provide users
%%more succinct information.
%%
%% Motivated by the scalability limitations of the approaches above, of
%% perfectly accurate decision sets, \cite{ilsms-aaai21} proposed a novel
%% two-stage approach to the decision set computation problem, where the
%% method exhaustively enumerates individual rules and then computes a
%% subset of rules agreeing with the training data.
%
%%
%% Compared with the other work~\cite{yisb-cp20}, the exhaustive rule
%% enumeration process leads to a dramatically more compact encoding,
%% which contributes to a more scalable method of decision set generation
%% problems.
%%
%% The second part can be considered as a set cover problem, where the
%% authors minimize either the number of rules or the number of literals
%% in the model with the use of integer linear programming.
%%
%
%Post-hoc explainability is one of the major approaches to XAI.
%%
%Besides a plethora of heuristic sampling-based approaches to post-hoc
%explainability~\cite{guestrin-kdd16,lundberg-nips17,guestrin-aaai18},
%a formal reasoning based method to computing abductive
%explanations~\cite{darwiche-ijcai18,inms-aaai19} stands out.
%%
%AXps can be related with prime implicants of the decision function
%(hence an alternative name \emph{prime implicant explanations},
%\emph{PI-explanations}) associated with ML predictions and so are
%guaranteed to capture the semantics of the ML models in the entire
%feature space.
%%
%Although hard to compute in general, AXps were shown to be effectively
%computable for BT models by an incremental MaxSAT-based
%approach~\cite{iisms-aaai22}.
%
%Our work aims at making a bridge between interpretable DS models and
%AXp computation by exploiting the latter for training the former.
%%
%In particular and given a BT model, it focuses on generating decision
%rules that agree with the BT.
%%
%Each decision rule represents an AXp for the prediction made by the BT
%model, resulting in a DS model in a way \emph{guided} by the original
%BT model.
%%
%The approach is shown to outperform the prior logic-based approaches
%to DS inference in terms of test accuracy and performance.


==> texfigs/bt.tex <==
%------------------------------------------------------------------------------%
% File:        bt.tex
%
% Description:
%
% Created:     7 Feb 2018.
%
% Author:      Alexey Ignatiev (aign).
%------------------------------------------------------------------------------%

% defining box structure
\tikzstyle{box} = [draw=black!90, thick, rectangle, rounded corners,
                     inner sep=10pt, inner ysep=20pt, dotted
                  ]
\tikzstyle{title} = [draw=black!90, fill=black!5, semithick, top color=white,
                     bottom color = black!5, text=black!90, rectangle,
                     font=\small, inner sep=2pt, minimum height=1.3em,
                     top color=tyellow2!27, bottom color=tyellow2!27
                    ]
% block styles
\tikzstyle{feature} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                       draw=black!80, top color=tblue2!20,bottom color=tblue2!25,%
                       draw, minimum height=1.1em, text centered,%
                       inner sep=2pt%
                      ]
\tikzstyle{pscore} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=tgreen3!20,bottom color=tgreen3!27,%
                     draw, minimum height=1.1em, text centered,%
                     inner sep=2pt%
                    ]
\tikzstyle{nscore} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=tred2!20,bottom color=tred2!25,%
                     draw, minimum height=1.1em, text centered,%
                     inner sep=2pt%
                    ]

\begin{adjustbox}{center}
\setlength{\tabcolsep}{3pt}
\def\arraystretch{3}
\begin{tabular}{ccc}
    \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.314\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{1}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (0.016, 0.57) {Status $=$ Married?};
        \node [feature, below left  = 0.8em and -2.78em of feat1] (feat2) {Education $=$ Dropout?};
        \node [feature, below right = 0.8em and -2.78em of feat1] (feat3) {Rel. $=$ Not-in-family?};

        % leaf nodes
        \node [nscore, below left  = 0.8em and -2.8em of feat2] (pos1) {-0.1569};
        \node [pscore, below right  = 0.8em and -2.8em of feat2] (neg1) {0.0770};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.1089};
        \node [nscore, below right = 0.8em and -2.8em of feat3] (neg2) {-0.3167};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    &
    \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.302\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{2}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (-0.335, 0.57) {Hours/w $\leq$ 40?};
        \node [feature, below left  = 0.8em and -2.36em of feat1] (feat2) {Status $=$ Married?};
        \node [feature, below right = 0.8em and -2.36em of feat1] (feat3) {Status $=$ Never-Married?};

        % leaf nodes
        \node [nscore, below left  = 0.8em and -2.8em of feat2] (pos1) {-0.0200};
        \node [nscore, below right  = 0.8em and -2.8em of feat2] (neg1) {-0.2404};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.1245};
        \node [pscore, below right = 0.8em and -2.8em of feat3] (neg2) {0.0486};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    &
     \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.28\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{3}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (0.113, 0.57) {Education $=$ Doctorate?};
        \node [feature, below left  = 0.8em and -3.6em of feat1] (feat2) {40 $<$ Hours/w $\leq$ 45?};
        \node [feature, below right = 0.8em and -3.6em of feat1] (feat3) {Rel. $=$ Own-child?};

        % leaf nodes
        \node [pscore, below left  = 0.8em and -2.8em of feat2] (pos1) {0.0605};
        \node [pscore, below right  = 0.8em and -2.8em of feat2] (neg1) {0.3890};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.2892};
        \node [nscore, below right = 0.8em and -2.8em of feat3] (neg2){-0.0580};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    \\
   \end{tabular}
\end{adjustbox}

%------------------------------------------------------------------------------%


